Hash-Based Tree Similarity and Simplification in Genetic Programming for Symbolic Regression

We introduce in this paper a runtime-efficient tree hashing algorithm for the identification of isomorphic subtrees, with two important applications in genetic programming for symbolic regression: fast, online calculation of population diversity and algebraic simplification of symbolic expression trees. Based on this hashing approach, we propose a simple diversity-preservation mechanism with promising results on a collection of symbolic regression benchmark problems.

==> fig/stats_various.tex <==
\begin{tabular}{m{2.5cm}m{2.3cm}p{2.3cm}p{2.3cm}r}
Problem data &                   Algorithm &  $R^2$ (training) &  $R^2$ (test) & Time (s) \\
 \midrule
     Breiman - I & GA           & 0.870 $\pm$ 0.040 & 0.865 $\pm$ 0.037 & 1084.5 \\
     Breiman - I & GA Diversity & 0.875 $\pm$ 0.034 & 0.870 $\pm$ 0.029 & 1207.5 \\
     Breiman - I & NSGA-2       & $\mathbf{0.885 \pm 0.013}$ & $\mathbf{0.879 \pm 0.012}$ & 1584.0 \\
% \midrule
    Friedman - I & GA           & 0.859 $\pm$ 0.007 & 0.860 $\pm$ 0.006 & 1090.5 \\
    Friedman - I & GA Diversity & 0.860 $\pm$ 0.007 & 0.860 $\pm$ 0.005 & 1207.0 \\
    Friedman - I & NSGA-2       & $\mathbf{0.863 \pm 0.002}$ & $\mathbf{0.863 \pm 0.003}$ & 1554.0 \\
% \midrule
   Friedman - II & GA           & 0.944 $\pm$ 0.038 & 0.942 $\pm$ 0.041 & 1092.0 \\
   Friedman - II & GA Diversity & 0.957 $\pm$ 0.023 & 0.957 $\pm$ 0.025 & 1248.0 \\
   Friedman - II & NSGA-2       & $\mathbf{0.958 \pm 0.008}$ & $\mathbf{0.957 \pm 0.010}$ & 1474.0 \\
% \midrule
         Pagie-1 & GA           & 0.990 $\pm$ 0.012 & 0.889 $\pm$ 0.107 & 442.5 \\
         Pagie-1 & GA Diversity & 0.994 $\pm$ 0.005 & 0.912 $\pm$ 0.070 & 540.5 \\
         Pagie-1 & NSGA-2       & $\mathbf{0.998 \pm 0.002}$ & $\mathbf{0.932 \pm 0.075}$ & 880.0 \\
% \midrule
         Poly-10 & GA           & 0.820 $\pm$ 0.293 & 0.764 $\pm$ 0.478 & 405.0 \\
         Poly-10 & GA Diversity & 0.840 $\pm$ 0.089 & 0.838 $\pm$ 0.120 & 518.0 \\
         Poly-10 & NSGA-2       & $\mathbf{0.879 \pm 0.072}$ & $\mathbf{0.850 \pm 0.099}$ & 902.5 \\
\end{tabular}


==> fig/stats_vladislavleva.tex <==
\begin{tabular}{m{2.5cm}m{2.3cm}p{2.3cm}p{2.3cm}r}
Problem data &                   Algorithm &  $R^2$ (training) &  $R^2$ (test) & Time (s) \\
 \midrule
 Vladislavleva-1 & GA           & 0.999 $\pm$ 0.001 & 0.946 $\pm$ 0.120 & 371.5 \\
 Vladislavleva-1 & GA Diversity & 0.999 $\pm$ 0.001 & 0.980 $\pm$ 0.106 & 450.0 \\
 Vladislavleva-1 & NSGA-2       & $\mathbf{1.000 \pm 0.000}$ & $\mathbf{0.987 \pm 0.026}$ & 784.5 \\
% \midrule
 Vladislavleva-2 & GA           & 0.995 $\pm$ 0.012 & 0.987 $\pm$ 0.028 & 355.0 \\
 Vladislavleva-2 & GA Diversity & 0.995 $\pm$ 0.012 & 0.992 $\pm$ 0.016 & 462.0 \\
 Vladislavleva-2 & NSGA-2       & $\mathbf{0.999 \pm 0.001}$ & $\mathbf{0.998 \pm 0.002}$ & 802.0 \\
% \midrule
 Vladislavleva-3 & GA           & 0.968 $\pm$ 0.062 & 0.932 $\pm$ 0.508 & 445.0 \\
 Vladislavleva-3 & GA Diversity & 0.979 $\pm$ 0.048 & 0.975 $\pm$ 0.053 & 570.0 \\
 Vladislavleva-3 & NSGA-2       & $\mathbf{0.995 \pm 0.014}$ & $\mathbf{0.989 \pm 0.042}$ & 920.5 \\
% \midrule
 Vladislavleva-4 & GA           & 0.951 $\pm$ 0.036 & 0.918 $\pm$ 0.053 & 527.0 \\
 Vladislavleva-4 & GA Diversity & 0.968 $\pm$ 0.023 & 0.936 $\pm$ 0.049 & 651.0 \\
 Vladislavleva-4 & NSGA-2       & $\mathbf{0.982 \pm 0.017}$ & $\mathbf{0.966 \pm 0.027}$ & 973.5 \\
% \midrule
 Vladislavleva-5 & GA           & 0.997 $\pm$ 0.012 & 0.933 $\pm$ 0.144 & 407.0 \\
 Vladislavleva-5 & GA Diversity & 0.999 $\pm$ 0.002 & 0.995 $\pm$ 0.015 & 502.5 \\
 Vladislavleva-5 & NSGA-2       & $\mathbf{1.000 \pm 0.000}$ & $\mathbf{0.997 \pm 0.023}$ & 871.0 \\
% \midrule
 Vladislavleva-6 & GA           & 0.869 $\pm$ 0.155 & 0.072 $\pm$ 0.329 & 369.0 \\
 Vladislavleva-6 & GA Diversity & 0.939 $\pm$ 0.143 & 0.255 $\pm$ 0.978 & 491.0 \\
 Vladislavleva-6 & NSGA-2       & $\mathbf{1.000 \pm 0.023}$ & $\mathbf{1.000 \pm 0.347}$ & 930.0 \\
% \midrule
 Vladislavleva-7 & GA           & 0.895 $\pm$ 0.048 & 0.878 $\pm$ 0.100 & 395.0 \\
 Vladislavleva-7 & GA Diversity & 0.904 $\pm$ 0.029 & 0.892 $\pm$ 0.058 & 501.5 \\
 Vladislavleva-7 & NSGA-2       & $\mathbf{0.917 \pm 0.017}$ & $\mathbf{0.899 \pm 0.033}$ & 843.5 \\
% \midrule
 Vladislavleva-8 & GA           & 0.962 $\pm$ 0.080 & 0.541 $\pm$ 0.569 & 362.5 \\
 Vladislavleva-8 & GA Diversity & 0.986 $\pm$ 0.033 & 0.787 $\pm$ 0.436 & 489.5 \\
 Vladislavleva-8 & NSGA-2       & $\mathbf{0.992 \pm 0.012}$ & $\mathbf{0.817 \pm 0.412}$ & 799.0 \\
\end{tabular}

